On Min-Cut Algorithms for Half-Duplex Relay Networks

Computing the cut-set bound in half-duplex relay networks is a challenging optimization problem, since it requires finding the cut-set optimal half-duplex schedule. This subproblem in general involves an exponential number of variables, since the number of ways to assign each node to either transmitter or receiver mode is exponential in the number of nodes. We present a general technique that takes advantage of specific structures in the topology of a given network and allows us to reduce the complexity of computing the half-duplex schedule that maximizes the cut-set bound (with i.i.d. input distribution). In certain classes of network topologies, our approach yields polynomial time algorithms. We use simulations to show running time improvements over alternative methods and compare the performance of various half-duplex scheduling approaches in different SNR regimes.

==> results.tex <==
% to help texshop compile main.tex
% !TEX root = main.tex


%\subsection{Description of Main Results}

In order to study the problem of finding the half-duplex schedule that maximizes the cut-set bound, we first set up the problem of maximizing the half-duplex cut-set bound as a linear optimization problem whose variables describe the half-duplex schedule.
This problem cannot be solved efficiently as a linear program since it involves an exponential number of variables and constraints.
The techniques introduced in \cite{PE11}, which exploit a submodularity property of mutual information, can be used to solve the optimization problem without evaluating each of the exponentially many cut-set constraints in the linear program.
However, we are still left with an exponential number of variables, reflecting the fact that, in a half-duplex network, the number of mode configurations is exponential in the number of nodes. As a result, even if we knew the solution to the optimization problem, the description of the optimal schedule would take exponentially large amounts of memory.

Our main result is a technique that allows exploiting specific
properties of the network topology to reduce the number of
variables in the linear program. This is done by showing that,
if the node set can be divided into smaller parts satisfying
certain properties, the probability distribution describing the
half-duplex schedule can be factorized into factors involving the nodes
in these parts.
More specifically, if we can find (possibly overlapping) subsets of nodes $V_1,V_2,...,V_k$ for some $k$ such that
\begin{itemize}
\item for any cut, the cut value is only a function of the local schedule at each of the $V_i$s,
\item given local schedules for each of the $V_i$s, a global schedule can be constructed,
\end{itemize}
then it is possible to find an equivalent formulation of the optimization problem involving a number of variables that is exponential on $\max_i |V_i|$.
Thus, provided that we can find subsets $V_1,...,V_k$ whose sizes are much smaller than the total number of nodes, the complexity reduction can be very significant.
For example, the line network considered in \cite{cheaprelay} is one special case where $V_1,V_2,...$ can be chosen as all pairs of consecutive nodes ($|V_i|=2$ for all $i$), and the problem of finding the half-duplex schedule that maximizes the cut-set bound (which, in this case, is actually capacity-optimal) can be solved in polynomial time in the size of the network.
The conditions that the $V_i$s need to satisfy will be made precise in Section \ref{mainsec}.


The remainder of the paper is organized as follows. 
In Section \ref{settingsec} we formally define the problem of optimizing the half-duplex schedule to maximize an approximation to the cut-set bound. 
We then introduce the intuition and main ideas used to solve the problem efficiently in Section \ref{examplesec}, by means of a simple example. 
In Section \ref{mainsec}, we use the intuition provided in the example to formalize the properties required from the node subsets $V_1,V_2,...,V_k$.
Then, in Section \ref{equivsec}, we state Theorem \ref{mainthm}, which provides an equivalent formulation of the half-duplex schedule optimization problem, for a given choice of node subsets $V_1,...,V_k$.
Sections \ref{equivproof} and \ref{computproof} contain the proof of Theorem \ref{mainthm}.
In Section \ref{heuristicsec}, we describe a heuristic for finding node subsets $V_1,...,V_k$ satisfying the required properties.
We then proceed to illustrating the usefulness of the result by employing it in two classes of network topologies.
These two classes can be seen as generalizing line networks in two different directions.
First, in Section \ref{layeredsec}, we consider layered networks, where the number of nodes per layer is at most logarithmic in the number of layers.
Then, in Section \ref{linesec}, we consider line networks where, in addition to an edge connecting every pair of consecutive nodes, there is an edge connecting nodes that are at a distance $2$ of each other, thus giving the network a non-layered topology.
For both of these classes, our technique allows the half-duplex schedule that maximizes the cut-set bound to be computed in polynomial time in the network size.
In Section \ref{extsec}, we briefly describe how our techniques can be extended to other network models.
We validate our results in Section \ref{sec:simulations} with a numerical analysis of our proposed algorithm compared to the current best known approach, which requires solving a problem with an exponential number of variables.
%We notice that, for small networks, the extra overhead required by our algorithm makes it slower than the simple brute force approach.
%However, as the number of nodes increases, 
We show that our algorithm significantly outperforms the brute force approach in networks of moderate and large size. 
We conclude our paper in Section \ref{sec:conc}.

